Anomaly Detection in Graph Structured Data: A Survey

Real-world graphs are complex to process for performing effective analysis, such as anomaly detection. However, recently, there have been several research efforts addressing the issues surrounding graph-based anomaly detection. In this paper, we discuss a comprehensive overview of anomaly detection techniques on graph data. We also discuss the various application domains which use those anomaly detection techniques. We present a new taxonomy that categorizes the different state-of-the-art anomaly detection methods based on assumptions and techniques. Within each category, we discuss the fundamental research ideas that have been done to improve anomaly detection. We further discuss the advantages and disadvantages of current anomaly detection techniques. Finally, we present potential future research directions in anomaly detection on graph-structured data.

==> anomalies/gradualAnomaly.tex <==
% \subsection{Gradual Anomalies}

==> anomalies/suddenAnomaly.tex <==
% \subsection{Sudden Anomalies}
% In real-time anomaly detection problem, many research papers primarily focus on detecting anomalous changes on graph such as bridge edges [22, 26], hotspot nodes [31], changes to community structure [27, 28], graph metrics [8, 10], etc.

% The anomaly detection technique in which they are focus on detecting anomalies involving the sudden appearance or disappearance of a large dense directed sub-graphs (near bi-cliques), which is useful in numerous applications: detecting attacks (port scan, denial of service) in network communication logs, interesting/fraudulent behavior creating spikes of activity in user-user communication logs (scammers who operate fast and in bulk), important events (holidays, large delays) creating abnormal traffic in/out flow to certain locations, etc. 

% We highlight two important aspects of the above definition. The (dis)appearance of a large dense sub-graph is anomalous only if it is sudden, i.e., it has not been observed before or is not part of a slow evolution (e.g., steadily growing communities). Similarly, the sudden (dis)appearance of a large number of edges is anomalous only if the edges form a dense sub-graph (the so-called lockstep behavior indicating fraud [5]). 
